Real-Time Incremental Explanations for Object Detectors in Autonomous Driving

Object detectors are widely used in safety-critical real-time applications such as autonomous driving. Explainability is especially important for safety-critical applications, and due to the variety of object detectors and their often proprietary nature, black-box explainability tools are needed. However, existing black-box explainability tools for AI models rely on multiple model calls, rendering them impractical for real-time use. In this paper, we introduce IncX, an algorithm and a tool for real-time black-box explainability for object detectors. The algorithm is based on linear transformations of saliency maps, producing sufficient explanations. We evaluate our implementation on four widely used video datasets of autonomous driving and demonstrate that IncX's explanations are comparable in quality to the state-of-the-art and are computed two orders of magnitude faster than the state-of-the-art, making them usable in real time.

==> explainability.tex <==
\subsection{Explainability}

Existing algorithms for explaining the output of image classifiers can be roughly divided into black-box algorithms, which are agnostic to the structure of the classifier, and white-box ones, which rely on the access to the internals of the classifier. There are clear advantages to the black-box tools, namely being agnostic to the internal structure and complexity of the classifier. Yet, black-box tools are in general much less efficient than white-box ones, as they rely on querying the classifier many times. Thus, they cannot be used as-is to explain the outputs of object detectors, whose main characteristic is efficiency.

There is a large body of work on algorithms for computing an explanation
for a given output of an image classifier. They can be largely grouped
into two categories: propagation and perturbation.  Propagation-based
explanation methods back-propagate a model's decision to the input
layer to determine the weight of each input
feature for the decision~\cite{springenberg2015striving,
sundararajan2017axiomatic, bach2015pixel, shrikumar2017learning,
nam2020relative}. \gradcam only needs
one backward pass and propagates the class-specific gradient into the final convolutional layer of a 
DNN to coarsely highlight important regions of an input image~\cite{CAM}. 

Perturbation-based explanation approaches introduce perturbations to the input space directly
in search for an explanation. \shap (SHapley Additive exPlanations) 
computes Shapley values of different parts of the input and uses them to rank the
features of the input according to their importance~\cite{lundberg2017unified}.
\lime constructs a small neural network to label the original input and its neighborhood of perturbed
images and uses this network to estimate the importance of different parts of the input
~\cite{lime, datta2016algorithmic,
chen2018learning, petsiuk2018rise, fong2019understanding}. 

Finally, Causal \underline{R}esponsibility \underline{eX}planations (\rex)~\cite{CKK23,CKS21} (formerly \deepcover) is an XAI tool 
based on the solid foundations of causal reasoning~\cite{Hal48}. 
Essentially, \rex constructs an approximation of a causal explanation~\cite{HP05,Hal48} by first ranking the pixels of a given image
according to their importance for the classification, and then constructing an explanation greedily from the saliency landscape of
the pixels. The ranking is an approximate degree of responsibility~\cite{CH04}, 
computed on the coarsely partitioned image, and updated by refining
the areas of the input with high responsibility, until a sufficiently fine partition is reached. 

To compute the degree of responsibility, \rex generates mutants -- images with some of the parts
masked -- and queries the classifier on these mutants. If a non-masked area is sufficient to get the same classification as the original
image, it is a cause for the classification, with the degree of responsibility of each part based on the number of parts in the area.
For example, if a part by itself is sufficient for the classification, the responsibility of each of its pixels is $1$; 
if, however, the smallest set of
parts needed to obtain the same classification is of size $5$, then each pixel in each part of this set has the responsibility $1/5$.

Essentially, the responsibility is in $[0,1]$, and the higher it is, the more important a given pixel is for the classification.
If a part has no influence on the classification, the responsibility of each of its pixel is $0$, and it is eliminated from further analysis.
The process is repeated over a number of different random partitions, and the result is averaged.

Most of the tools mentioned above do not work with \yolo, or any object detector, natively.
There exists a version of \gradcam for \yolo~\cite{gradcamyolo}; unfortunately, however, it is proprietary and not available for experiments. 


==> reproducibility.tex <==
\section{Reproducibility Checklist}

This paper:
\begin{itemize}
\item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes/partial/no/NA)  \textbf{YES}
\item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no)    \textbf{YES}
\item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes/no)   \textbf{YES}
\item Does this paper make theoretical contributions? (yes/no)  \textbf{YES}
\end{itemize}

If yes, please complete the list below.

\begin{itemize}
\item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)    \textbf{YES}
\item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)  \textbf{YES}
\item Proofs of all novel claims are included. (yes/partial/no) \textbf{YES}
\item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no) \textbf{YES}
\item Appropriate citations to theoretical tools used are given. (yes/partial/no)   \textbf{YES}
\item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)  \textbf{YES}
\item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)   \textbf{YES}
\item Does this paper rely on one or more datasets? (yes/no)    \textbf{YES}
\end{itemize}

If yes, please complete the list below.

\begin{itemize}
\item A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA)  \textbf{YES}
\item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA)  \textbf{YES}
\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA)    \textbf{YES}
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA)  \textbf{YES}
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA)    \textbf{YES}
\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA)    \textbf{YES}
\item Does this paper include computational experiments? (yes/no)   \textbf{YES}
\end{itemize}

If yes, please complete the list below.

\begin{itemize}
\item Any code required for pre-processing data is included in the appendix. (yes/partial/no)  \textbf{YES}
\item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no)    \textbf{YES}
\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no) \textbf{YES}
\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no) \textbf{YES}
\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA)   \textbf{YES}
\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no)  \textbf{YES}
\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no)    \textbf{YES}
\item This paper states the number of algorithm runs used to compute each reported result. (yes/no) \textbf{YES}
\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no)   \textbf{YES}
\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no)   \textbf{YES}
\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA)   \textbf{YES}
\item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA)   \textbf{YES}
\end{itemize}
